EXPLORA: Efficient Exemplar Subset Selection for Complex Reasoning

Answering reasoning-based complex questions over text and hybrid sources, including tables, is a challenging task. Recent advances in large language models (LLMs) have enabled in-context learning (ICL), allowing LLMs to acquire proficiency in a specific task using only a few demonstration samples (exemplars). A critical challenge in ICL is the selection of optimal exemplars, which can be either task-specific (static) or test-example-specific (dynamic). Static exemplars provide faster inference times and increased robustness across a distribution of test examples. In this paper, we propose an algorithm for static exemplar subset selection for complex reasoning tasks. We introduce EXPLORA, a novel exploration method designed to estimate the parameters of the scoring function, which evaluates exemplar subsets without incorporating confidence information. EXPLORA significantly reduces the number of LLM calls to ~11% of those required by state-of-the-art methods and achieves a substantial performance improvement of 12.24%. We open-source our code and data (https://github.com/kiranpurohit/EXPLORA).

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% \color{purple}
% Is our method specific to in-context numerical reasoning, or can it also work for other NLU tasks? What is special about numerical reasoning? Can we say that we design a general method but test it on numerical reasoning tasks because they are more difficult? \color{green} As semantic similarity between train and test set can't be used to select ICEs in case of numerical reasoning. Therefore we propose EXPLORA.\\
% \color{black}
% \color{blue}
% - We are given only the task-specific loss, which is different from generative model error. We do not utilize the logits given by generative models. Bayesian explanation, in-context one iteration GD -- each of these papers, can we say why these theories don't apply to complex QA.

% Complex numerical reasoning tasks such as financial question answering \cite{chen2022finqa} or tabular question answering \cite{tabmwp} require both language understanding as well as reasoning skills.
% Large language models (LLMs) have been shown to exhibit both these skills.
% Language understanding skills help  While 

% \color{gray}

Answering complex questions that require multi-step numerical reasoning \cite{chen2022finqa,tabmwp,aqua_rat,roy2016solving} over structured and unstructured sources is an active research area with applications in finance, law, and healthcare~\cite{wang2023survey}.
% The complexity in such tasks could arise from multiple factors, such as the need to parse heterogeneous sources like tables and text \cite{chen2022finqa} coupled with multi-step numerical reasoning \cite{tabmwp,aqua_rat,roy2016solving} to answer the question. 

Existing supervised approaches for numerical reasoning involve fine-tuning of multiple generative models for generating arithmetic programs or stepwise solution to the original problem \cite{chiang-chen-2019-semantically,amini-etal-2019-mathqa,aqua_rat,roy2016solving,geva-etal-2020-injecting,cobbe2021training}. 
 
% However, existing approaches require expensive annotations of supervised stepwise rationales along with the solution for fine-tuning multiple generative models \cite{aqua_rat} \cite{cobbe2021training} \cite{geva-etal-2020-injecting} lacking a general purpose solution. 

\begin{figure*}[t]
\centering

\includegraphics[width=0.8\textwidth]{figures/explora-cropped.pdf}\\
\caption{Overview of \static{}, proposed exemplar selection approach.}
\label{fig:icl}
% \vspace{-4mm}
\end{figure*}


More recently, the advances in Large Language Models (LLMs) has lead to substantial progress in a wide range of natural language understanding and reasoning tasks \cite{brown2020gpt3}. The emergent capabilities in LLMs\cite{wei2022emergent,gpt3incontext} such as In-Context Learning (ICL) has paved the way to a new class of approaches that employ chain-of-thought reasoning~\cite{complex_cot} \cite{wei2023chainofthought} for solving complex numerical reasoning questions.
Instead of fine-tuning task-specific models, these approaches focus on choosing carefully constructed exemplars with rationales to be used as input to LLMs, commonly termed as prompting.
% A distinct advantage of prompting with demonstration samples vs fine-tuning is  that the LLM is a general-purpose machine that can be used to solve multiple numerical reasoning tasks.
% In this paper, our focus is to propose a general framework that can be employed to solve multiple QA tasks that require numerical reasoning over homogeneous and heterogeneous sources by selecting suitable demonstration samples.

\mpara{The limitations of manual exemplar selection.} 
% It is inherently hard for the LLMs to perform multi-step reasoning using few-shot in-context learning with just the  \texttt{(input, output)} pairs~\cite{rae2022scaling}.
To tackle complex numerical reasoning problems, \textit{chain-of-thought} (COT) prompting was proposed to add hand-crafted natural language rationales (stepwise solutions) to the prompts in addition to input and output resulting in \texttt{(input, rationale, output)}~\cite{wei2023chainofthought}.
% The process of generating stepwise natural language rationales can be seen as decomposing the original problem to simpler problems that can be solved with less effort \cite{wei2023chainofthought} \cite{brown2020gpt3}.

% Interesting, 
% COT rationales for compositional natural language questions involve generating explanations for the final answer. 
% However, such explanations have been found to be unfaithful to the reasoning process of underlying LLM \cite{turpin2023language,ye2022unreliability} for answering compositional questions in complex QA, unlike numerical reasoning questions. 
% In such cases, the decomposition of such question to simpler sub-questions is observed to be more faithful. To induce such decomposition capabilities in LLMs, authors of the work self-ask \cite{self_ask} modify COT prompting and propose to add hand-crafted follow-up questions derived from the original complex questions to the prompt.
However, there are inherent limitations of COT approach for complex and hybrid numerical reasoning tasks. 
The COT involves the manual effort of selecting the best exemplars with appropriate rationales that sufficiently convey the  execution strategy for the task under consideration. The manual selection process is tedious and not scalable across different numerical reasoning tasks. Since the outputs generated by the LLM are highly sensitive to exemplars provided \cite{lu-etal-2022-fantastically,zhao2021calibrate,chang2023data}, it is crucial to select meaningful exemplars that are robust across evaluation samples and improve overall task performance.

\mpara{Limitations of automated exemplar selection approaches}:
To tackle these limitations, several automated exemplar selection approaches have been proposed \cite{ye2023compositional,lu-etal-2022-fantastically,rubin-etal-2022-learning,complex_cot}. These approaches are usually dynamic exemplar selection methods, which select several demonstration examples from the training set for each test example. Several approaches also require annotated data and training of several models for exemplar selection\cite{lu2023dynamic,ye2023compositional}. These approaches entail to heavy computational requirements during inference, especially when there is a large pool of exemplars to select from. While unsupervised approaches like similarity \cite{rubin-etal-2022-learning} or diversity based \cite{ye-etal-2023-complementary} approaches exist for dynamic exemplar selection, they also require projecting the input query and the entire pool of exemplars to a continuous vector space followed by search, increasing computational time during inference. Additionally, the majority of these approaches assume the exemplars chosen to be independent of each other and only consider the interaction between the test sample and the exemplars. They do not account for the interactions between the exemplars themselves.

 As an alternative to dynamic exemplar selection approaches, LENS \cite{li2023finding} proposed to select a static set of task level support exemplars. However, LENS assumes access to language model output logits and involves multiple expensive evaluations of the LLM for scoring the exemplars. LENS also does not model the interactions between exemplars and scores each sample independently. 
% In the example below, using Few-shot-COT results in inaccurate results due to lack of decomposition information in its prompt (hidden due to space reasons).
% \input{intro-example-mouth}

\mpara{\static{} (Static Exemplar Selection Approach):}
In this work, we propose a novel static exemplar selection method \static{}, that selects multiple high value/low loss exemplar subsets. An overview of the working of \static{} is shown in Figure \ref{fig:icl}. The selection of task level exemplar subsets are performed once, and we model the interactions between exemplars through initial sampling of subsets and by directly scoring and selecting subsets. We propose a parameterized scoring function that approximates the loss indicative of task performance using features from a transformer based embedding model. We propose an exploration mechanism as shown in Figure \ref{fig:icl} to estimate the parameters of the scoring function with minimal calls to the LLM and without access to logits from the LLM. Our approach mitigates the expensive processing during inference incurred by traditional dynamic exemplar selection approaches and obviates the need for manual exemplar selection while providing high performance.


\mpara{Contributions.} The core contributions of our work are:
\begin{description}
    \item 
    1) We propose a new robust static exemplar selection approach \static{}, that selects task level exemplars for numerical reasoning based questions.

    \item 
    2) We demonstrate the ability of transferring selected exemplars across models. We show that exemplars selected using smaller models can be used to induce reasoning capabilities in much larger models leading to reduced costs.
     \item 
     3) We demonstrate that \static{} is less resource intensive compared to existing approaches, as it results in minimal calls to the LLMs for exemplar selection.
    \item 
    4) We conduct extensive experiments with different exemplar selection methods to showcase the generalized performance of \static{} across multiple complex and hybrid numerical reasoning based QA tasks.
\end{description}

\color{black}


==> table-qualitative.tex <==



\begin{table*}
\begin{tabular}{lp{.80\textwidth}}
\toprule
    \textbf{Method}     & \textbf{Decomposition} \\
\midrule


\colorg \textbf{Question}  & \colorg \textbf{In 2010 and 2009 , what was the total fair value in billions of assets segregated for the benefit of securities and futures brokerage customers?} [Dataset: \textbf{FinQA}] \\
\COT{}  & To find the total fair value in billions of assets segregated for the benefit of securities and futures brokerage customers in 2010 and 2009, we need to look at the table. \textcolor{red}{In 2010, the fair value was \$25.0 billion and in 2009, it was \$24.0 billion. Hence total is \textbf{Answer:} \$49 billion.}  \\
\colorg \icat{} + \ftd{} & \colorg \textbf{Rationale:} To find the total fair value in billions [\dots], look at the table for the years 2010 and 2009. In the table, under "year ended December 31," we can see two columns [\dots], there is a row labeled "securities and futures brokerage customers." In this row, there are values listed in millions.To convert these values to billions, we divide each value by 1000.
\textcolor{teal}{For 2010: \$25.0 billion (segregated cash) + \$9.7 billion (fair value of securities) = \$34.7 billion
For 2009: \$24.0 billion (segregated cash) + \$10.2 billion (fair value of securities) = \$34.2 billion
[\dots] \textbf{Answer:} 68.9}
 \\
\icat{} & in billions, we need to look at Note 29 in the text. 
In 2010, \$25.0 billion in cash and \$9.7 billion in securities with [\dots]. 
In 2009, \$24.0 billion in cash and \$10.2 billion in securities [\dots].
\textbf{Answer}: \texttt{68.9 (billion)}. \\
\midrule
\midrule


\end{tabular}
\caption{Qualitative analysis of reasoning chains generated by chain-of-thought vs \icat{}}
\label{tab:qualitative}
%\vspace{-0.25cm}
\end{table*}



==> table-results-llm-calls.tex <==
\begin{table*}[t]
    \centering
    % resizebox{\textwidth}{!}{% 
    \begin{tabular}{lccccccc}
    \toprule

\textbf{Datasets} & \textbf{\begin{tabular}[c]{@{}c@{}}Zero-Shot \\ COT\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Few-Shot\\  COT\end{tabular}} & \textbf{Random} & \textbf{KNN}  & \textbf{MMR}  & \textbf{LENS} & \textbf{Explora} \\
    
     % \textbf{Datasets}& \multicolumn{1}{c}{\textbf{Zero-Shot COT}}& \multicolumn{1}{c}{\textbf{Few-shot COT}} & \multicolumn{1}{c}{\textbf{Random}} & \multicolumn{1}{c}{\textbf{KNN}} & \multicolumn{1}{c}{\textbf{MMR}} & \multicolumn{1}{c}{\textbf{LENS}} & \multicolumn{1}{c}{\textbf{Explora}}  \\
    

    \midrule

    \textbf{GSM8K}    &1319   &1319   &1319   &1319    &1319    &24176     &4719   \\
    \textbf{AquaRat}  &254    &254    &254    &254     &254     &23111     &3654   \\
    \textbf{TabMWP}   &7686   &7686   &7686   &7686    &7686    &30543     &11086  \\
    \textbf{FinQA}    &1147   &1147   &1147   &1147    &1147    &24004     &4547   \\
      \bottomrule
    \end{tabular}
    % } 
    \caption{Frugal subset selection approach - we reduce number of calls to LLMs. Our score based approach enables us to make fewer calls to LLMs compared to LENS which lacks this score based modelling.}
    % \vspace{-1cm}
    \label{tab:llm_calls}
\end{table*}


==> table-results-v2.tex <==
\begin{table*}[!t]
    \centering
    
    \begin{tabular}{lcccc}
    \toprule
    
     \textbf{Method}& \multicolumn{1}{c}{\aqua{}}& \multicolumn{1}{c}{\strat{}} & \multicolumn{1}{c}{\advhotpot{}} & \multicolumn{1}{c}{\tab{}}  \\
     
     % & cover-EM & cover-EM& EM& EM&EM \\
    %  \midrule
    %  \fshot{}& 11.66& 28.41& 85.74& 78.2& 42.55\\
     
    %  \COT{} &20.85& 34.08&94.79&  79.4&52.22 \\
     
    %  \zfshot{} & 12.22& 19.25& 88.75& 75.4& 47.51 \\
    % \hline
    % \self{} & 23.64& 32.58& N/A& N/A& N/A \\
      
    %   \autocot{} &  N/A& N/A&  93.83 & 76.2 & N/A \\

        \midrule
    
    SOTA & \bf \colorit 37.60  & \colorit  \bf 50.59 &   60.5  &  47.3 \\
    
        \midrule
 \colorg \textbf{gpt-3.5-turbo} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


        \midrule
 \colorg \textbf{Mistral} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\


      \midrule
\colorg \textbf{Llama-2-7B} &\colorg & \colorg& \colorg& \colorg\\

   random&  24.36& 29.41&  92.95 &   77.60  \\

    \mmr+\selfcon{}  &  26.99& 30.69&  \coloritt  95.13 & \colorit  80.70  \\
    
     \static{}+\selfcon{}  &  27.07& 30.33&  94.96 & \colorit  80.70  \\
     
    \static{}+\pot{}+\selfcon{} &  \coloritt  \textbf{27.24}$\ddagger$& \coloritt  \textbf{36.00}&  \colorit  \textbf{96.14}$\dagger$ & \colorit  \textbf{80.70}  \\



        \midrule
 \colorg \textbf{FLAN-T5-XL} & \colorg& \colorg& \colorg& \colorg\\
  
    random &  20.28& 25.33&  81.71 & 74.7  \\
    
    \mmr{}+\selfcon{} &  1.59 & 20.00 &  10.25 & 8.31  \\
      
    \static{}+\selfcon{} &  25.24$\dagger$&  34.00& \colorit  96.14 $\dagger$ & \coloritt  80.0  \\
      
    \static{}+\pot{}+\selfcon{} &  24.92$\dagger$&  34.00& \colorit   $\dagger$ & \coloritt     \\
     
     \bottomrule
    \end{tabular}
    \caption{Results across datasets. $\dagger$ and $\ddagger$ indicates statistical significance over \COT{} at 0.1 level  and 0.01 level respectively. SOTA results are included for completion.}
    % \vspace{-1cm}
    \label{tab:main_result}
\end{table*}

